URSABench: Comprehensive Benchmarking of Approximate Bayesian Inference Methods for Deep Neural Networks

While deep learning methods continue to improve in predictive accuracy on a wide range of application domains, significant issues remain with other aspects of their performance including their ability to quantify uncertainty and their robustness. Recent advances in approximate Bayesian inference hold significant promise for addressing these concerns, but the computational scalability of these methods can be problematic when applied to large-scale models. In this paper, we describe initial work on the development ofURSABench(the Uncertainty, Robustness, Scalability, and Accu-racy Benchmark), an open-source suite of bench-marking tools for comprehensive assessment of approximate Bayesian inference methods with a focus on deep learning-based classification tasks

==> methods.tex <==
%!TEX root = main.tex
\section{Methods}
\label{sec:methods}

\section{The {\acro} Framework}

The \texttt{\acro} framework is split into modules in order to abstract each component to the user:
\begin{itemize}
    \item \textbf{Inference class:} receives a single set of hyperparameters, a model, and a data set. Materialises samples via the \texttt{sample} method or in an iterative manner via \texttt{sample\_iterative}. Examples are the \texttt{HMC} class and the \texttt{SGLD} class.
    \item \textbf{Task class:} is initialised with a data set and once instantiated, operates on a set of samples provided by an \texttt{Inference} object. Examples are the \texttt{Prediction} class and the \texttt{OODDetection} class.
    \item \textbf{Hyperparameter Optimization class:} receives the task over which to evaluate, as well as the inference scheme and its corresponding hyperparameter domain. Examples are the \texttt{BayesOpt} class and the \texttt{RandomSearch} class.
    \item \textbf{Workflow template:} Structures the modules to be run in a convenient Python script.
\end{itemize}
This modular form is designed to enable others to contribute to any single part of the workflow. For example, rather than assessing the performance of approximate Bayesian inference methods, one could focus on comparing and improving on the hyperparameter optimization module.

\paragraph{Hyperparameter Optimization:} A key focus of this framework is to incorporate the cost of optimizing over the hyperparameters for each Monte Carlo method. Although less glamorous, hyperparameter optimization can be the determinant of whether or not to opt for an inference technique. For example, if we are resource constrained or using a cloud infrastructure, it is necessary to have some notion of the time it will take to achieve a certain level of performance. Approximate inference approaches that either require searching over a high-dimensional hyperparameter space or are sensitive to certain settings can perform poorly if the available resources are limited. Therefore \texttt{\acro} is a benchmark framework that includes hyperparameter optimization and we can gather metrics such as wall-clock time and number of evaluations until a certain level of performance. In \texttt{\acro} we include grid search, random search, and Bayesian optimization, where we rely on \texttt{BoTorch} \cite{} for Bayesian optimization. 

\paragraph{Uncertainty Tasks:} Designing the right tasks to quantify the uncertainty performance of different inference schemes across multiple models is challenging as different behaviours are desirable depending on the task. We tend to use metrics that aim to capture certain characteristics of the predictive distribution, without fully being able to assess the entire quality of the approximation. As an example, accuracy may be a good indicator that the distribution has converged to suitable mode, but as many previous works in the literature have shown, this may not be useful for determining the performance for data set distribution shifts or for out of distribution samples. Therefore, our framework has focused on three specific tasks to study the quality of the materialized samples. As is consistent with the literature, we have included an OOD task and an ID task. Furthermore, we offer an additional decision-making task that is targeted at measuring the quality in the tail of the predictive distribution. In particular, we enforce data sets to have classes that are of high priority, yet to appear less frequently. We design cost matrices to penalise misclassifications on these rare high priority classes and then compare inference schemes by the cost ensued from the decisons taken. This idea is similar to that taken by \cite{cobb2018loss} for measuring performance.

\paragraph{Metric:} \textcolor{red}{Some comment on metrics. Ideally a comment on timing / calibration function for resource cost}

\paragraph{Inference with MCMC:} Previous works that have aimed at providing benchmarks for BNNs have mostly focused on variational inference (VI) \cite{google,gal}. This is mostly due to the success of scaling VI to large NN models. On the other hand, MCMC approaches to inference in BNNs have seen fewer appearances in benchmarks, despite starting to gain a lot of traction in the field. Hence, the focus of \texttt{\acro} is to benchmark recent MCMC approximate inference schemes, whilst allowing others to easily add their own. 


% have a high dimensional search space in the number of hyperparameters can take longer to optimise over unless 


% This less glamorous part of most 


% Although this procedure is often forgotten when introducing a new approximate inference technique, 

% a vital test of a new method is how easy it is to tune to a task. Therefore we provide the user with the ability to measure the time taken to perform 

% \usepackage{graphicx}
% \usepackage{subcaption}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{images/HypOpt.pdf}
        \caption{Workflow for hyperparameter optimization.}
        \label{fig:gull}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{images/Job.pdf}
        \caption{Workflow for uncertainty quantification tasks.}
        \label{fig:tiger}
    \end{subfigure}
    \caption{Summary of module interactions.}
\end{figure}
